Improving Prototypical Parts Abstraction for Case-Based Reasoning Explanations Designed for the Kidney Stone Type Recognition

The in-vivo identification of the kidney stone types during an ureteroscopy would be a major medical advance in urology, as it could reduce the time of the tedious renal calculi extraction process, while diminishing infection risks. Furthermore, such an automated procedure would make possible to prescribe anti-recurrence treatments immediately. Nowadays, only few experienced urologists are able to recognize the kidney stone types in the images of the videos displayed on a screen during the endoscopy. Thus, several deep learning (DL) models have recently been proposed to automatically recognize the kidney stone types using ureteroscopic images. However, these DL models are of black box nature whicl limits their applicability in clinical settings. This contribution proposes a case-based reasoning DL model which uses prototypical parts (PPs) and generates local and global descriptors. The PPs encode for each class (i.e., kidney stone type) visual feature information (hue, saturation, intensity and textures) similar to that used by biologists. The PPs are optimally generated due a new loss function used during the model training. Moreover, the local and global descriptors of PPs allow to explain the decisions ("what" information, "where in the images") in an understandable way for biologists and urologists. The proposed DL model has been tested on a database including images of the six most widespread kidney stone types. The overall average classification accuracy was 90.37. When comparing this results with that of the eight other DL models of the kidney stone state-of-the-art, it can be seen that the valuable gain in explanability was not reached at the expense of accuracy which was even slightly increased with respect to that (88.2) of the best method of the literature. These promising and interpretable results also encourage urologists to put their trust in AI-based solutions.

==> Apendix_A.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textcolor{green}{The following text is taken as reference from: \\ https://arxiv.org/pdf/2305.09062 }

\textcolor{gray}{
\subsubsection{Designing the ICNN Score}
In order to build and understand the Inter/Intra Class Nearest Neighbors Distance Score (ICNN Score), it is necessary to define the concepts of inter-class distance and intra-class distance \cite{james2013introduction}. The main idea for inter-class distance is that different classes should be distant or optimal with respect to a distance $d$ (Eq. \ref{GeneralInterClassDistance}),
\begin{equation}
D^*\left( C_i, C_j \right) = \sup_d
\frac{1}{n_i n_j} \sum_{x_j, x_k \in C_i}  d\left( x_j,  x_k \right), \label{GeneralInterClassDistance}
\end{equation}
which basically represents an average of the maximal distance matrix between elements of the two classes $i$ and $j$. 
In a similar way, the optimal intra-class distance is defined as
\begin{equation}
I^* \left( l_i \right) = \inf_d \frac{1}{n_i} \sum_{k_1=1}^{n_i} \sum_{k_2=k_1+1}^{n_i} d\left( x_{i, k_1},  x_{j,k_2} \right).
\end{equation}
}
\textcolor{gray}{
These quantities represent the distance between different classes and the density of those classes, respectively. Although these equations represent the basic ideas of inter- and intra-class distances, they are useful to develop a score that can be transformed into a loss function. For this, we propose a function that minimizes penalization to the neighborhood class elements to a particular sample $x_i \in C_j$. In addition, we also define a function that maximizes the penalization of elements $x_k \notin C_j$ to such sample $x_i$ based on their distance proximity.  In the ideal case with respect to $x_i$ at its neighborhood, the distances of elements in the same class are close to zero. In addition,  elements in the same neighborhood but in different classes than $x_i$, their distances to it are as large as possible. 
%(Figure \ref{fig:NeighborhoodICNNScore}). 
The former bound is easy to control and has the tendency to zero. However, the latter bound can be problematic, given the different distances that can be obtained. Thus, instead of having any large random possible distances, we force the bound of these distances to a known constant.
For this purpose,} \textcolor{cyan}{
we define the following neighborhoods: $N_{x_i}$ the $k$-nearest neighbors of  $x_i$ at the same class, and $N_{\tilde{x}_i}$ the $k$-nearest neighbors of $x_i$ at different classes.
}\textcolor{gray}{ Using these sets, it is possible to define the following function  based on a differentiable distance $d\left( x_i, x_j \right)$,
\begin{align}
 \alpha \left( x_i \right) = \max \left\{ d\left( x_i, p \right) \vert p \in N_{x_i} \cup N_{\tilde{x}_i} \right\} 
\end{align}
We also have the distance function,
\begin{equation}
  \theta \left( x_i \right) = \min \left\{ d\left( x_i, p \right) \vert p \in N_{x_i} \cup N_{\tilde{x}_i} \right\} 
\end{equation}
Using these functions, we define a normalization of the distances for all the elements in the neighborhood of $x_i$:
\begin{equation}
 h \left( x_i, p \right) = \frac{d\left( x_i, p \right) - \theta\left( x_i \right) }{ \alpha\left( x_i \right) - \theta\left( x_i \right)},
\end{equation}
\textcolor{gray}{which is a min-max normalization that enforces the desired bounds in the interval $[0,1]$. Now, we define a penalization $\lambda$ function for defining the concept of "far" or "near" to a specific $x_i$:}
\begin{align}
    \lambda_{\tilde{x}} \left( x_i \right) & = \sum_{p\in N_{\tilde{x}_i}} h \left( x_i, p \right) \label{TotalNormDistanceNotClass}, \\
    \lambda_{x} \left( x_i \right) & = \sum_{p\in N_{x_i}} \left[ 1-h\left( x_i, p \right) \right] \label{TotalNormDistanceClass}
\end{align}
}

\textcolor{gray}{
The first equation (Eq. \ref{TotalNormDistanceNotClass}) represents the normalized penalization of the elements in a certain neighborhood of elements in different classes than the class of $x_i$, and the second equation represents a similarity to elements at $N_{x_i}$. Therefore, we have
\begin{align}
    \lambda\left( x_i \right) = \frac{\lambda_{\tilde{x}} \left( x_i \right) + \lambda_{x} \left( x_i \right) }{\left|N_{\tilde{x}_i} \cup N_{x_i}  \right|}
    \label{Lambda:BeforeFixing}
\end{align}
Thus, if we want to maximize this function, the average $\lambda_{\tilde{x}}/N$, with $N=\left|N_{\tilde{x}_i} \cup N_{x_i}  \right|$, needs to be maximized. Thus, the distances of the elements not belonging to the class of $x_i$ are maximized to it. In the case of $\lambda_{x}/N$, the similarities are maximized toward one, thus forcing the elements belonging to the class of $x_i$ to get near to it or to zero. However, when going through the battery of experiments, a change is proposed on the original $\lambda$ function (Eq. \ref{Lambda:BeforeFixing}) to improve results for the few-shot learning setup,
\begin{equation}
    \lambda \left( x_i \right) = \frac{\lambda_{\tilde{x}} \left( x_i \right)}{\left|N_{\tilde{x}_i}\right|} + \frac{\lambda_{x} \left( x_i \right)}{\left| N_{x_i}  \right|}.
\end{equation}
Therefore, we have that each of $\lambda's$ $x$ functions finish as
 \begin{align}
     \frac{\lambda_{\tilde{x}} \left( x_i \right)}{\left|N_{\tilde{x}_i}\right|} & \thickapprox E_{h}  \left[ h\left( x_i , p \right) \vert p \in N_{\tilde{x}_i} \right],  \nonumber \\
         \frac{\lambda_{x} \left( x_i \right)}{\left| N_{x_i}  \right|} & \thickapprox 1 -  E_{h} \left[ h\left( x_i , p \right) \vert p \in N_{x_i} \right]  \nonumber.
 \end{align} 
\noindent These expected values depend on the original distribution of the $d\left( x_i, p \right)$ given that we have a uniform a priori, and the likelihood of the defined distance. Now, if the $\lambda$ function is maximized with respect to the representation of $x_i$ and $p$, two phenomena occur: First, the inter-distance on $N_{x_i}$ is minimized, and second, the intra-distance on $N_{\tilde{x}_i}$ is maximized. This basically corresponds to highly dense and compact class clusters with large distances between them, our ideal case for classification. Therefore, integrating this $\lambda$ function to a cost function will enforce these properties in the generated embedding during the learning process of a neural network. }
 
 \textcolor{gray}{
%\begin{proposition}\label{Proposition1}
\textbf{Proposition:}\textit{
Given the $\lambda$ function and a smooth embedding representation for the samples $x_i$ based on weights $\mathcal{F}$. If $\lambda$ is maximized by using a gradient method on those weights, the embedding will change to increase the inter-class distance and minimize the intra-class distance at the classes.}
%\end{proposition}
%\begin{proof}
%Appendix \ref{Proof:Proposition1}
%\end{proof}
%\noident 
This proposition allows to say that a cost function based on the ICNN  helps to separate the class clusters when training on data. Next, given that we have  $h\left(x_i \right)\leq 1$, if we add overall terms $i$, we finish with
\begin{align}
    \sum_{p\in N_{\tilde{x}_i}} h\left(x_i, p \right) & \leq \left| N_{\tilde{x_i}} \right| \longrightarrow \frac{\lambda_{\tilde{x}}\left( x_i \right)}{\left| N_{\tilde{x_i}} \right|} \leq 1
\end{align}
In a similar way, $0 \leq \frac{\lambda_x \left( x_i \right) }{ \left| N_{x_i} \right|}\leq 1$ given that also $h\left(x_i , p\right) \leq 1$ for $p \in N_{\tilde{x}} \cup N_{x}$. In this way, $ 0 \leq \lambda \left( x_i \right) \leq 2$.\\
Now, we would like to avoid large changes while learning the distances between elements in the neighborhood of $x_i$. For this, we introduce a penalization function over the terms $h$ that minimizes the possible variance (Eq. \ref{VarianceDistanceMinimization}).
\begin{equation}
    \omega \left( x_i \right) = \alpha - \left[ Var\left( \lambda_{\tilde{x}} \left( x_i \right)  \right) +  Var\left( \lambda_{x}\left( x_i \right)  \right) \right]
    \label{VarianceDistanceMinimization}
\end{equation}
}
\textcolor{gray}{
%\noident 
The variance of this function depends on the original distribution of values $d\left( x_i, p \right)$. \\
%\begin{proposition}\label{Proposition2}
\textbf{Proposition: }
\textit{
Given the $\omega$ function and the smooth embedding representation based on weights $\mathcal{F}$. If the loss function is minimized, the $\omega$ is maximized by using the gradient method on those weights, then the inter and intra-class variances can be minimized by selecting an adequate $alpha$. \\
}
%\end{proposition}
%\begin{proof}
%Appendix \ref{Proof:Proposition2}
%\end{proof
%\noident 
Thus, optimizing a loss function based on the ICNN helps to minimize the variance of the learned manifold or in other words it favors dense clusters. In order to obtain the bounds for $\omega$, we can use a classic definition of variance,
\begin{align*}
    Var\left( \lambda_{\tilde{x}} \left( x \right) \right)
    & = E \left( \lambda_{\tilde{x}}^2 \left( x \right) \right) - E^2\left[ \lambda_{\tilde{x}} \left( x \right) \right]
\end{align*}
\noindent
Thus, 
\begin{align*}
    E\left[ \lambda_{\tilde{x}}\left(x \right) \right] & \thickapprox \frac{1}{\left|X \right|} \sum_{x\in X} \lambda_{\tilde{x}} \left( x \right) \\
    & \thickapprox  \frac{1}{\left|X \right|} \sum_{x\in X} \sum_{p\in N_{\tilde{x}}} h \left( x, p \right) 
\end{align*}
\noindent In this way, we have that the variance is bounded as
\begin{align*}
    Var\left( \lambda_{\tilde{x}} \left( x \right) \right) \leq & 
     \frac{1}{\left|X \right|} \sum_{x\in X} \left( \sum_{p\in N_{\tilde{x}} }  h \left( x, p \right) \right)^2 -...\\
     & \left( \max_{x_i} \left| N_{\tilde{x}_i} \right| \right)^2 \\
     \leq &   \frac{1}{\left|X \right|} \sum_{x\in X} \left( \sum_{p\in N_{\tilde{x}} }  h \left( x, p \right) \right)^2 \\
     & - \left( \max_{x_i} \left| N_{\tilde{x}} \right| \right)^2 \leq k_1^2,
 \end{align*}
where $k_1 = \max_{x_i} \left| N_{\tilde{x}} \right|$
 This $k_1$ happens when all the elements at $N_{\tilde{x}}$ have a distance of one. In a similar way, we have $Var\left( \lambda_{x} \left( x \right) \right) \leq k_2^2$ which is also  $k_2 = \max_{x_i} \left| N_{x} \right|$
 In the reverse case, we have that 
the lower bound for both variances is 0.
 In this way, we have that we can use $\omega = k_1^2+k_2^2$ to go force the best case where $x$ has the maximal separation from elements not in the class and minimal separation from elements in the same class. }

\textcolor{gray}{
Finally, we have the last penalization for the ICNN Score which represents how many elements in the neighborhood  $N_{\tilde{x}_i} \cup N_{x_i} $ belong  to the same class as $x_i$,
\begin{equation}
    \gamma \left( x_i \right) = \frac{\left| N_{x_i}  \right|}{\left| N_{x_i}  \right|+\left| N_{\tilde{x_i}}  \right|}
\end{equation}
Therefore, using these three functions, it is possible to build the ICCNScore,
\begin{equation}
    ICNN\left(X\right) = \frac{1}{\left| X \right|}  \sum_{x_i \in X} \lambda\left(x_i\right)^{\frac{1}{p}} \omega\left(x_i\right)^{\frac{1}{q}} \gamma\left(x_i\right)^{\frac{1}{r}}
\end{equation}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/Backbone_vs_PPs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Comparison of ProtoPNet using different CNN architectures as the feature extractor against the pure finetuned CNN, with Data Augmentation (DA) and without Data Augmentation (NoDA)}
\label{Backbone_vs_PPs}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\multirow{2}{*}{} & \multicolumn{2}{c}{DenseNet201} & \multicolumn{2}{c}{ResNet50} & \multicolumn{2}{c}{VGG16} \\
     & CNN    & PPs    & CNN    & PPs    & CNN    & PPs    \\ \hline
NoDA & 79.2\% & 84.1\% & 76.0\% & 83.1\% & 85.0\% & 76.9\% \\
DA   & 89.4\% & 85.5\% & 85.0\% & 85.9\% & 84.0\% & 81.0\%
\end{tabular}%
}
\end{table}

==> tables/Deletion_Boxplots_example.tex <==
\begin{figure}[ht] 
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/deletion_ProtoPNet_vs_backbone_DenseNet201_long.pdf}
    \caption{\small{
    %Deletion scores per class comparing ProtoPNet heatmaps (in blue) against Grad-CAMs from its backbone (in orange). 
    Comparison of "deletion" scores by class of the heat maps obtained from a ProtoPnet, against those from GradCAM of a CNN. Both the ProtoPNet backbone and the separately trained CNN are a DenseNet201 convolutional architecture.
    In this case, ProtoPNet uses 3 prototypical parts per class and both networks are trained with data augmentation as described in section  \ref{Implementation_Details}. 
    It is observed, \textit{deletion} average ProtoPNet scores outperform GradCAMs, for three classes (WW, BRU, CYS). ProtoPNet "deletion" scores also present a reduced variability than the results presented by GradCAM, hence a more consistent behavior when generating .
    Classes WW, WD, AU, STR, BRU and CYS are described in section \ref{Kidney_stone_dataset}.
    %The classes observed are WW (Whewellite, type Ia), WD (Weddellite, type IIa), AU (Acide Urique, type IIIa), STR (Struvite, type IVc), BRU (Brushite, type IVd), CYS (Cystine, type Va).
    Image best seen in color.
    }}
    \label{fig:umaps}
\end{figure}

==> tables/Descriptors_example1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{}
\label{Descriptors_example1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc}
\multicolumn{3}{c}{Highest activated Prototypical-Part: 13th}                                                                                          \\ \hline
Descriptor & \begin{tabular}[c]{@{}c@{}}Local\\      Activation \%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Global \\      Activation \%\end{tabular} \\ \hline
Hue        & 62.2\% & 33.6\% \\
Texture    & 60.7\% & 31.4\% \\
Contrast   & 57.6\% & 24.7\% \\
Shape      & 57.3\% & 23.5\% \\
Brightness & 49.7\% & 15.3\% \\
Saturation & 29.9\% & 15.0\% \\ \hline
Avg        & 52.9\% & 23.9\%
\end{tabular}%
}
\end{table}

==> tables/ProtoPNet_diff_backbones_and_classes_Accu.tex <==
\begin{table*}[!h]
\centering
%\resizebox{\linewidth}{!}{%
\scalebox{1.0}{\begin{tabular}{@{}ccccccccccccc@{}}
%\toprule
%\begin{tabular}{cccccccccc}
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ProtoPNet   \\      with backbone:\end{tabular}} &
  \multicolumn{3}{c}{Accuracy 4 classes} &
  \multicolumn{3}{c}{Accuracy 5 classes} &
  \multicolumn{3}{c}{Accuracy 6 classes} \\
 &
  Surface &
  Section &
  Mixed &
  Surface &
  Section &
  Mixed &
  Surface &
  Section &
  Mixed \\ \hline
Resnet18 &
  87.37\% &
  79.62\% &
  83.13\% &
  \textbf{89.00\%} &
  79.70\% &
  84.95\% &
  \textbf{81.17\%} &
  70.50\% &
  76.12\% \\
Resnet50 &
  89.75\% &
  74.88\% &
  84.94\% &
  85.20\% &
  \textbf{81.40\%} &
  84.10\% &
  80.08\% &
  \textbf{72.17\%} &
  76.46\% \\
Resnet152 &
  87.00\% &
  \textbf{80.50\%} &
  \textbf{85.25\%} &
  81.20\% &
  81.30\% &
  \textbf{85.60\%} &
  77.17\% &
  \textbf{72.17\%} &
  77.29\% \\
VGG16 &
  89.75\% &
  73.62\% &
  84.94\% &
  87.60\% &
  75.80\% &
  84.05\% &
  75.50\% &
  70.58\% &
  75.08\% \\
VGG19 &
  \textbf{92.00\%} &
  75.25\% &
  83.87\% &
  82.40\% &
  74.80\% &
  82.95\% &
  78.08\% &
  69.33\% &
  74.58\% \\
DenseNet201 &
  89.75\% &
  80.00\% &
  81.69\% &
  86.90\% &
  79.00\% &
  85.35\% &
  79.42\% &
  70.50\% &
  \textbf{77.88\%}
\end{tabular}
}
\caption{Test Accuracy for different ProtoPNet Backbones and number of classes}
\label{table:Backbones_varingClassw}
\end{table*}


==> tables/SOTA_tab.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{
Accuracy of state-of-the-art models and three of ours for identifying kidney stones. Models trained with data augmentation.}
\label{table_SOTA_vs_ours}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
\multicolumn{2}{c}{\textbf{Method}}            & \textbf{Surface}  & \textbf{Section} & \textbf{Mixed} \\ \hline
\multicolumn{2}{c}{Martinez, et al. \cite{martinez2020towards}} & 56.2±23.3  & 46.6±12.8           & 52.7±18.9  \\
\multicolumn{2}{c}{Estrade, et al. \cite{Towards_autoKSclass_Vincent2021}}  & 73.7±17.9  & 78.8±10.6           & 70.1±22.3  \\
\multicolumn{2}{c}{Black, et al.\cite{black2020deep}}    & 73.5±19.0  & 88.8±02.8            & 80.1±13.8  \\
\multicolumn{2}{c}{Lopez, et al.\cite{lopez_AssessingDL_KSclass}}    & 81.0±03.0   & 88.0±02.3            & 85.0±03.0   \\
\multicolumn{2}{c}{Lopez, et al.\cite{lopez_tiro2022boosting}}    & 83.2±01.2   & 90.4±04.8            & 85.6±00.1   \\
\multicolumn{2}{c}{Villalvazo-Avila, et   al.\cite{VillalvazoAvila2022_ImprovedKS}} & \textbf{88.8±02.8} & 84.4±06.0         & \textbf{96.6±00.5}        \\ \hline
\multirow{3}{*}{Ours}   & Densenet201 3pps    & 80.2±00.6        & 87.6±06.2       & 85.2±01.5               \\
           & Resnet50 1pps           & 80.9±01.3 & \textbf{91.0±03.3} & 88.2±02.1 \\
           & Vgg16 10pps             & 76.7±02.2 & 82.6±04.9          & 82.1±00.9 \\ \hline
\end{tabular}%
}
\end{table}




==> tables/SOTA_vs_ProtoPNets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{
Accuracy of state-of-the-art models and three of ours for identifying kidney stones. Models trained with data augmentation.}
\label{table_SOTA_vs_ours}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
\multicolumn{2}{c}{\textbf{Method}}            & \textbf{Surface}  & \textbf{Section} & \textbf{Mixed} \\ \hline
\multicolumn{2}{c}{Martinez, et al. \cite{martinez2020towards}} & 56.2±23.3  & 46.6±12.8           & 52.7±18.9  \\
\multicolumn{2}{c}{Estrade, et al. \cite{Towards_autoKSclass_Vincent2021}}  & 73.7±17.9  & 78.8±10.6           & 70.1±22.3  \\
\multicolumn{2}{c}{Black, et al.\cite{black2020deep}}    & 73.5±19.0  & 88.8±02.8            & 80.1±13.8  \\
\multicolumn{2}{c}{Lopez, et al.\cite{lopez_AssessingDL_KSclass}}    & 81.0±03.0   & 88.0±02.3            & 85.0±03.0   \\
\multicolumn{2}{c}{Lopez, et al.\cite{lopez_tiro2022boosting}}    & 83.2±01.2   & 90.4±04.8            & 85.6±00.1   \\
\multicolumn{2}{c}{Villalvazo-Avila, et   al.\cite{VillalvazoAvila2022_ImprovedKS}} & \textbf{88.8±02.8} & 84.4±06.0         & \textbf{96.6±00.5}        \\ \hline
\multirow{3}{*}{Ours}   & Densenet201 3pps    & 80.2±00.6        & 87.6±06.2       & 85.2±01.5               \\
           & Resnet50 1pps           & 80.9±01.3 & \textbf{91.0±03.3} & 88.2±02.1 \\
           & Vgg16 10pps             & 76.7±02.2 & 82.6±04.9          & 82.1±00.9 \\ \hline
\end{tabular}%
}
\end{table*}


==> tables/Table_Accu_per_Training_Loss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{Table of accuracy scores for the different configurations of the ProtoPNet architecture trained with different loss functions. Additionally, the rightmost column presents the accuracy obtained with the considered black-box CNN used as the backbone for each of the configurations. All the models were trained over the Mixed kidney stone dataset.}
\label{table_accuracy_Losses_Functions}
\begin{tabular}{ccccccc}
\multicolumn{2}{c}{}                                                                                  & \multicolumn{4}{c}{ProtoPNet models}                                                                                                                                                                                                             & CNN models                  \\ \cline{3-7} 
\multicolumn{1}{l}{Backbone}                      & \multicolumn{1}{l}{\# of PPs}                     & CE Loss             & \begin{tabular}[c]{@{}c@{}}ProtoPNet   Loss\\      (ε = 0.0001)\end{tabular} & \begin{tabular}[c]{@{}c@{}}ProtoPNet   Loss\\      (ε = 0.01)\end{tabular} & \begin{tabular}[c]{@{}c@{}}CE + ICNN \\      Loss\end{tabular} & CE Loss                     \\ \hline
\multirow{5}{*}{Vgg16}                            & 1pps                                              & 81.71±1.88          & 81.78±1.60                                                                   & \textbf{84.27±0.90}                                                        & 82.59±1.55                                                     & \multirow{5}{*}{81.47±2.72} \\
                                                  & 3pps                                              & 82.75±2.78          & 82.21±3.33                                                                   & \textbf{83.91±1.44}                                                        & 83.72±1.54                                                     &                             \\
                                                  & 10pps                                             & \textbf{83.72±2.57} & 82.08±0.90                                                                   & 81.98±3.49                                                                 & 82.98±1.74                                                     &                             \\
                                                  & 50pps                                             & 82.06±1.47          & 82.61±1.95                                                                   & 82.39±1.48                                                                 & \textbf{83.27±2.72}                                            &                             \\
                                                  & 100pps                                            & \textbf{84.18±1.77} & 79.70±3.20                                                                   & 82.5±2.69                                                                  & 82.22±1.54                                                     &                             \\ \hline
\multirow{5}{*}{Resnet50}                         & 1pps                                              & 87.42±1.83          & \textbf{88.21±2.07}                                                          & 86.48±2.34                                                                 & 87.40±1.72                                                     & \multirow{5}{*}{83.40±5.32} \\
                                                  & 3pps                                              & 89.65±2.11          & 86.66±1.37                                                                   & 87.67±1.54                                                                 & \textbf{90.37±0.58}                                            &                             \\
                                                  & 10pps                                             & 89.50±0.78          & 85.44±1.44                                                                   & 86.40±1.31                                                                 & \textbf{89.98±1.09}                                            &                             \\
                                                  & 50pps                                             & 89.12±0.85          & 85.25±2.15                                                                   & 88.28±1.50                                                                 & \textbf{90.32±0.80}                                            &                             \\
                                                  & 100pps                                            & 90.02±0.86          & 86.52±1.42                                                                   & 86.77±3.00                                                                 & \textbf{90.20±0.67}                                            &                             \\ \hline
\multirow{5}{*}{DenseNet201}                      & 1pps                                              & 86.27±1.79          & 86.29±1.91                                                                   & \textbf{88.36±2.80}                                                        & 86.89±1.60                                                     & \multirow{5}{*}{89.67±3.60} \\
                                                  & 3pps                                              & \textbf{88.02±1.99} & 85.19±1.50                                                                   & 86.02±1.69                                                                 & 86.96±2.59                                                     &                             \\
                                                  & 10pps                                             & 88.48±1.37          & 87.29±0.92                                                                   & 87.81±2.12                                                                 & \textbf{89.84±0.72}                                            &                             \\
                                                  & 50pps                                             & 87.34±1.97          & 85.39±1.08                                                                   & 86.14±2.37                                                                 & \textbf{89.07±1.01}                                            &                             \\
                                                  & 100pps                                            & 88.23±1.07          & 83.62±3.18                                                                   & 85.89±1.77                                                                 & \textbf{88.53±2.80}                                            &                             \\ \hline
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Average Accuracy \\      per Training Loss\end{tabular}} & 86.56±3.25          & 85.02±2.83                                                                   & 85.66±2.85                                                                 & \textbf{86.96±3.42}                                            & 84.84±5.29                  \\ \hline
\end{tabular}
\end{table*}


==> tables/Table_accu_perclass_SOTA.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%--------------------------------------------
%--------------------------------------------
%--------------------------------------------
\begin{table*}[h]
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Reference} & \multicolumn{6}{c|}{Precision Per Class} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Weighted \\ Precision\end{tabular}} & \multirow{2}{*}{ML Method} \\ \cline{2-7}
 & AU & WW & WD & STR & CYS & BRU &  &  \\ \hline
{}\cite{serrat2017}{} & 0.65 & 0.55 & 0.69 & 0.50 & N/A & N/A & 0.63 & Random Forest \\ \hline
{}\cite{torrell}{} & 0.76 & 0.67 & 0.80 & 071 & N/A & 0.72 & 0.74 & Siamese CNN \\ \hline
{}\cite{black2020}{} & 0.94 & 0.95 & N/A & 0.71 & 0.75 & 0.75 & 0.85 & CNN – ResNet101 \\ \hline
\cite{martinez2020}& 0.91 & 0.94 & 0.92 & N/A & N/A & N/A & 0.92 & Random Forest \\ \hline
\cite{estrade2021} & 0.99 & 0.90 & 0.93 & N/A & N/A & N/A & 0.94 & ResNet152v2 \\ \hline
\cite{lopez2021assessing} & 0.99 & 0.90 & 0.93 & N/A & N/A & N/A & 0.94 & ResNet152v2 \\ \hline
\end{tabular}
\caption{Comparison of the  precision obtained by the three main contributions for the most common kidney stone classes. The precision is given for each individual class and classifier. The taxonomy per stone class same as in Table \ref{table_pworks1}. The average precision (weighted by the image number of each class) are also given for each kidney stone type. In the last table line, the precision values are given for surface images. For section images, the authors in \cite{estrade2021}, reported a precision of 0.95, 0.94 and 0.94 for AU, WW and WD, respectively. The corresponding weighted precision equals 0.94.}
\label{pworks2}
\end{table*}
%--------------------------------------------
%--------------------------------------------
%--------------------------------------------

==> tables/Table_simplified_urinary.tex <==
\begin{table*}[!h]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\bf{Type} & \bf{Acronym} & \bf{Occurrences} & \bf{Crystal shape} \\ \hline
Type I = Whewellite  & WW & from 15 up to 35 \% & Dumbbell shape \\ \hline
Type II = Weddellite & WD & from 15 up to 35 \% & Bipyramidal \\ \hline
Type IIIb = Uric Acid dihydrate & UA & from 2 up to 13 \%& Flat rhomboidal \\ \hline

Type IVc = Struvite & STR & from 20 up to 30 \% & Rectangular Prism \\ \hline
Type IVd = Brushite & BRU & from 5 up to 20 \%& Elongate narrow \\ \hline
Type V = Cystine & CYS & from 1 up to 3 \%& Hexagonal plates \\ \hline
\end{tabular}
\caption{Simplified urinary calculi classification:  the frequency of appearance and a description of the crystal morphology are given for each stone type.}
\label{Table_ks_class}
\end{table*}

==> tables/concordance_old_table.tex <==
%
%\begin{table*}[!t]
%\center
%\begin{tabular}{|l|l|l|l|l|l|l|}
%\hline
%Component & Stone type & \begin{tabular}[c]{@{}l@{}}\% Correct Matches\end{tabular} & \begin{tabular}[c]{@{}l@{}}Number of    \\ occurrences\end{tabular} & AUC & \begin{tabular}[c]{@{}l@{}}Precision\\  (PPV)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Recall\\(Sensitivity) \end{tabular} \\ \hline
%Whewellite & Ia or Ib & 85\% & 205 & 0.87 & 0.88 & 0.85 \\ \hline
%Weddellite & IIa or IIb & 85\% & 178 & 0.87 & 0.86 & 0.85 \\ \hline
%Uric Acid & IIIa or IIIb & 91\% & 64 & 0.95 & 0.94 & 0.91 \\ \hline
%Carbapatite & IVa & 81\% & 176 & 0.86 & 0.88 & 0.81 \\ \hline
%Struvite & IVc & 50\% & 10 & 0.74 & 0.45 & 0.50 \\ \hline
%Brushite & IVd & 65\% & 23 & 0.82 & 0.83 & 0.65 \\ \hline
%Cystine & Va & 100\% & 7 & N/A & N/A & N/A \\ \hline
%\end{tabular}
%\caption{
%\textcolor{blue}{OMIT -- }
%Matched results between endoscopic and microscopic studies. ``N/A'' stands for not applicable  and refers to data which are insufficient for a statistical use. This simplified class representation was adapted from \cite{estrade2021}}
%\label{concordance}
%\end{table*}
%

==> tables/cvpr22_simpleTable.tex <==
\begin{table*}[]
\centering
\caption{\small{Weighted average metrics comparison for section, surface, and mixed patches. ProtoPNet with VGG19 with batch normalization as the backbone (PPN-VGG19bn). VGG 19-layer model, configuration `E', with batch normalization (VGG19bn).
}}
\label{tab:my-table}
\scalebox{0.88}{\begin{tabular}{@{}ccccccccccccc@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Precision} & \multicolumn{3}{c}{Recall} & \multicolumn{3}{c}{F1 score} \\ \cmidrule(l){2-13} 
                       & Surface  & Section  & Mixed  & Surface   & Section  & Mixed  & Surface  & Section & Mixed & Surface  & Section  & Mixed  \\ \midrule
PPN-VGG19bn            & 0.98     & 0.99     & 0.97   & 0.98      & 0.99     & 0.97   &
 0.98     & 0.99    & 0.97  & 0.98     & 0.99     & 0.97   \\
VGG19bn                & 0.99     & 1.00     & 1.00   & 0.99      & 1.00     & 1.00   & 0.99     & 1.00    & 1.00  & 0.99     & 1.00     & 1.00   \\
AlexNet                & 0.96     & 0.97     & 0.97   & 0.96      & 0.97     & 0.97   & 0.96     & 0.97    & 0.97  & 0.96     & 0.97     & 0.97   \\ \bottomrule
\end{tabular}
}
\end{table*}

==> tables/prior-works.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Overview of the kidney stone classes and acquisition conditions in the-state-of-the-art works, as well as for this contribution.  Simplified taxonomy: UA: Uric Acid (Anhydrous and Dihydrate), COM: Calcium Oxalate Monohydrate (whewellite, WW), COD: Calcium Oxalate Dihydrate (weddellite, WD), STR: Struvite, CYS: Cystine, BRU: Brushite.}
\label{table_pworks1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{rccccccccc}
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Reference / Feature}}} &
  \multicolumn{6}{c}{\textbf{Kidney stone composition}} &
  \multicolumn{2}{c}{\textbf{Image Type}} &
  \multicolumn{1}{l}{\multirow{2}{*}{Adquisition}} \\
\multicolumn{1}{c}{} &
  \textbf{AU} &
  \textbf{WW} &
  \textbf{WD} &
  \textbf{STR} &
  \textbf{CYS} &
  \textbf{BRU} &
  \textbf{Surface} &
  \textbf{Section} &
  \multicolumn{1}{l}{} \\
Serrat et al. (2017)                              & ✓ & ✓ & ✓ & ✓                    & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & ✓ & ✓ & Ex-vivo         \\
Torrell et al. (2018)                             & ✓ & ✓ & ✓ & ✓                    & \multicolumn{1}{l}{} & ✓                    & ✓ &   & Ex-vivo         \\
Black et al. (2020)                               & ✓ & ✓ &   & ✓                    & ✓                    & ✓                    & ✓ & ✓ & Ex-vivo         \\
Martinez et al. (2020)                            & ✓ & ✓ & ✓ & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & ✓ & ✓ & In-vivo         \\
Estrade et al. (2021)                             & ✓ & ✓ & ✓ & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & ✓ & ✓ & In-vivo         \\
Lopez et al. (2021)                               & ✓ & ✓ & ✓ & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & ✓                    & ✓ & ✓ & In-vivo         \\
Ochoa-Ruiz et al. (2022)                          & ✓ & ✓ & ✓ & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & ✓ & ✓ & In-vivo         \\
Villlalvazo-Avila et al. (2022)                   & ✓ & ✓ & ✓ & ✓                    & ✓                    & ✓                    & ✓ & ✓ & Ex-vivo         \\
Flores-Araiza et al. (2022)                       & ✓ & ✓ & ✓ & ✓                    & ✓                    & ✓                    & ✓ & ✓ & Ex-vivo         \\
Mendez-Ruiz et al. (2022)                         & ✓ & ✓ & ✓ & ✓                    & ✓                    & ✓                    & ✓ & ✓ & In-vivo/Ex-vivo \\
Lopez-Tiro et al. (2022)                          & ✓ & ✓ & ✓ & ✓                    & ✓                    & ✓                    & ✓ & ✓ & Ex-vivo         \\
Villalvazo-Avila et al. (2023)                    & ✓ & ✓ & ✓ & ✓                    & ✓                    & ✓                    & ✓ & ✓ & Ex-vivo         \\
Lopez-Tiro et al. (2023)                          & ✓ & ✓ & ✓ & ✓                    & ✓                    & ✓                    & ✓ & ✓ & Ex-vivo         \\
Flores-Araiza et al. (2023)                       & ✓ & ✓ & ✓ & ✓                    & ✓                    & ✓                    & ✓ & ✓ & Ex-vivo         \\
\multicolumn{1}{c}{Gonzalez-Zapata et al. (2023)} & ✓ & ✓ & ✓ & ✓                    & ✓                    & ✓                    & ✓ & ✓ & Ex-vivo         \\
\multicolumn{1}{c}{This contribution}             & ✓ & ✓ & ✓ & ✓                    & ✓                    & ✓                    & ✓ & ✓ & Ex-vivo        
\end{tabular}%
}
\end{table*}




\begin{table*}[h]
\centering
\arrayrulecolor{black}
\begin{tabular}{!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}} 
\hline
\multirow{2}{*}{Reference/Feature} & \multicolumn{6}{l!{\color{black}\vrule}}{Kidney Stone Composition} & \multicolumn{2}{l!{\color{black}\vrule}}{Image Type} & \multirow{2}{*}{Acquisition}  \\ 
\cline{2-9}
                                   & AU         & WW         & WD          & STR         & CYS           & BRU           & Surface        & Section  &          \\ 
\hline
{}\cite{serrat2017}              & \ding{51}  & \ding{51}   & \ding{51}    & \ding{51}   &  &                  & \ding{51}    &  \ding{51}        &      Ex vivo     \\ 
\cline{1-1}
{}\cite{torrell}             & \ding{51}  & \ding{51}   & \ding{51}    & \ding{51}   &     & \ding{51}   & \ding{51}      &           &    Ex vivo        \\ 
\cline{1-1} 
{}\cite{black2020}              & \ding{51}  & \ding{51}   &              & \ding{51}   & \ding{51}      & \ding{51}    & \ding{51}      & \ding{51}  &   Ex vivo          \\ 
\cline{1-1}
{}\cite{martinez2020}               &         \ding{51}  & \ding{51}   &  \ding{51}       &   &     &    &  \ding{51}    & \ding{51}  &   In vivo          \\ 
\cline{1-1}
{}\cite{estrade2021}               &         \ding{51}  & \ding{51}   &  \ding{51}       &   &     &    &  \ding{51}    & \ding{51}  &   In vivo          \\ 
\cline{1-1}
{}\cite{lopez2021assessing}               &         \ding{51}  & \ding{51}   &  \ding{51}       &   &     &   \ding{51}  &  \ding{51}    & \ding{51}  &   In vivo          \\ 
\cline{1-1}
{}\cite{estrade2021}               &         \ding{51}  & \ding{51}   &  \ding{51}       &   &     &    &  \ding{51}    & \ding{51}  &   In vivo          \\ 
\cline{1-1}
{}\cite{ochoa_ruiz2022vivo}               &         \ding{51}  & \ding{51}   &  \ding{51}       &   &     &    &  \ding{51}    & \ding{51}  &   In vivo          \\ 
\cline{1-1}
This contribution                               & \ding{51}  & \ding{51}   & \ding{51}     &  \ding{51}     & \ding{51}  & \ding{51}    & \ding{51}       &  \ding{51}        &           In vivo           \\
\hline
\end{tabular}
\arrayrulecolor{black}
\caption{Overview of the kidney stone classes and acquisition conditions in the-state-of-the-art works, as well as for this contribution.  Simplified taxonomy: UA: Uric Acid (Anhydrous and Dihydrate), COM: Calcium Oxalate Monohydrate (whewellite, WW), COD: Calcium Oxalate Dihydrate (weddellite, WD), STR: Struvite, CYS: Cystine, BRU: Brushite.
\textcolor{blue}{add most recent works of Francisco}
}
\label{table_pworks1}
\end{table*}


==> tables/tab9.tex <==
\begin{table*}[]
\footnotesize
% Different letter sizes:
%\tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, 
%\Large, \LARGE, \huge, and \Huge
\centering
\caption{Comparison of the implemented baselines, SOTA PrtotoPNet variants and our implementations.}
\label{tab_base_n_sota}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccccccc}
 &
   &
   &
  \multicolumn{3}{c}{IID} &
   &
  \multicolumn{3}{c}{OOD} \\
\multicolumn{3}{c}{Training   configuration:} &
  Accuracy (\%) &
  Precision (\%) &
  F1 (\%) &
   &
  Accuracy (\%) &
  Precision (\%) &
  F1 (\%) \\
\multicolumn{3}{c}{DenseNet201} &
  \textbf{89.67±3.60} &
  \textbf{90.51±3.60} &
  \textbf{89.47±3.46} &
   &
  \textbf{58.44±28.06} &
  60.22±29.62 &
  \textbf{54.54±32.73} \\
\multicolumn{3}{c}{ResNet50} &
  83.40±5.32 &
  85.58±4.30 &
  83.11±5.21 &
   &
  45.12±20.82 &
  49.16±24.08 &
  38.25±23.47 \\
\multicolumn{3}{c}{Vgg16} &
  81.47±2.72 &
  84.71±2.64 &
  80.62±3.84 &
   &
  58.35±22.62 &
  \textbf{63.73±19.93} &
  54.38±26.30 \\
\multicolumn{3}{c}{\textbf{CNNs (Baseline)   Average}} &
  84.84±5.29 &
  86.93±4.35 &
  84.4±5.60 &
   &
  53.97±24.62 &
  57.70±25.40 &
  49.06±28.56 \\
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}ProtoPool\\      (Improved backpropagation)\end{tabular}} &
   &
   &
   &
   &
   &
   &
   \\
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Proto2Proto\\      (Meta-PPs)\end{tabular}} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
   &
   &
   &
   \\
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}EvalProtoPNet\\      (Robust ProtoPNet)\end{tabular}} &
   &
   &
   &
   &
   &
   &
   \\
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Deformable\\      (Improved PPs vectors)\end{tabular}} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} \\
\multicolumn{3}{c}{\textbf{SOTA Average}} &
  84.55±2.98 &
  85.46±2.78 &
  84.49±3.09 &
   &
  56.88±20.53 &
  63.46±17.61 &
  53.38±23.69 \\
\multirow{5}{*}{ProtoPNet Loss} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}DenseNet201\\      + ResNet50\\      + Vgg16\end{tabular}} &
  1 &
   &
   &
   &
   &
   &
   &
   \\
 &
   &
  3 &
   &
   &
   &
   &
   &
   &
   \\
 &
   &
  10 &
   &
   &
   &
   &
  \textbf{} &
  \textbf{} &
  \textbf{} \\
 &
   &
  50 &
   &
   &
   &
   &
   &
   &
   \\
 &
   &
  100 &
   &
   &
   &
   &
   &
   &
   \\
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}ProtoPNet Loss\\      + ICNN\end{tabular}} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}DenseNet201\\      + ResNet50\\      + Vgg16\end{tabular}} &
  1 &
   &
   &
   &
   &
   &
   &
   \\
 &
   &
  3 &
   &
   &
   &
   &
   &
   &
   \\
 &
   &
  10 &
   &
   &
   &
   &
  \textbf{} &
  \textbf{} &
  \textbf{} \\
 &
   &
  50 &
   &
   &
   &
   &
   &
   &
   \\
 &
   &
  100 &
   &
   &
   &
   &
   &
   &
   \\
\multicolumn{3}{c}{\textbf{ProtoPNets Average}} &
  84.55±2.98 &
  85.46±2.78 &
  84.49±3.09 &
   &
  56.88±20.53 &
  63.46±17.61 &
  53.38±23.69
\end{tabular}%
%}
\end{table*}

==> tables/table_Accuracies_internal_val.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
\multicolumn{2}{c}{}                  & \multicolumn{4}{c}{ProtoPNet models}                                                  & CNN models                  \\ \hline
\multicolumn{1}{l}{Backbone} &
  \multicolumn{1}{l}{\# of PPs} &
  \begin{tabular}[c]{@{}c@{}}Accuracy   with\\      CE Loss\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Accuracy   with\\      ProtoPNet Loss\\      (ε = 0.0001)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Accuracy   with\\      ProtoPNet Loss\\      (ε = 0.01)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Accuracy   with\\      CE + ICNN \\      Loss\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Accuracy   with\\      CE Loss\end{tabular} \\ \hline
\multirow{5}{*}{Vgg16}       & 1pps   & 81.71±1.88          & 81.78±1.60          & \textbf{84.27±0.90} & 82.59±1.55          & \multirow{5}{*}{81.47±2.72} \\
                             & 3pps   & 82.75±2.78          & 82.21±3.33          & \textbf{83.91±1.44} & 83.72±1.54          &                             \\
                             & 10pps  & \textbf{83.72±2.57} & 82.08±0.90          & 81.98±3.49          & 82.98±1.74          &                             \\
                             & 50pps  & 82.06±1.47          & 82.61±1.95          & 82.39±1.48          & \textbf{83.27±2.72} &                             \\
                             & 100pps & \textbf{84.18±1.77} & 79.70±3.20          & 82.5±2.69           & 82.22±1.54          &                             \\ \hline
\multirow{5}{*}{Resnet50}    & 1pps   & 87.42±1.83          & \textbf{88.21±2.07} & 86.48±2.34          & 87.40±1.72          & \multirow{5}{*}{83.40±5.32} \\
                             & 3pps   & 89.65±2.11          & 86.66±1.37          & 87.67±1.54          & \textbf{90.37±0.58} &                             \\
                             & 10pps  & 89.50±0.78          & 85.44±1.44          & 86.40±1.31          & \textbf{89.98±1.09} &                             \\
                             & 50pps  & 89.12±0.85          & 85.25±2.15          & 88.28±1.50          & \textbf{90.32±0.80} &                             \\
                             & 100pps & 90.02±0.86          & 86.52±1.42          & 86.77±3.00          & \textbf{90.20±0.67} &                             \\ \hline
\multirow{5}{*}{DenseNet201} & 1pps   & 86.27±1.79          & 86.29±1.91          & \textbf{88.36±2.80} & 86.89±1.60          & \multirow{5}{*}{89.67±3.60} \\
                             & 3pps   & \textbf{88.02±1.99} & 85.19±1.50          & 86.02±1.69          & 86.96±2.59          &                             \\
                             & 10pps  & 88.48±1.37          & 87.29±0.92          & 87.81±2.12          & \textbf{89.84±0.72} &                             \\
                             & 50pps  & 87.34±1.97          & 85.39±1.08          & 86.14±2.37          & \textbf{89.07±1.01} &                             \\
                             & 100pps & 88.23±1.07          & 83.62±3.18          & 85.89±1.77          & \textbf{88.53±2.80} &                             \\ \hline
\multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Averag Accuracy \\      per Training Loss\end{tabular}} &
  86.56±3.25 &
  85.02±2.83 &
  85.66±2.85 &
  \textbf{86.96±3.42} &
  84.84±5.29 \\ \hline
\end{tabular}%
}
\caption{Accuracy scores for the different configurations of the ProtoPNet architecture trained with different loss functions. Additionally,
the rightmost column presents the accuracy obtained with the considered black-box CNN used as the backbone for each of
the configurations. All the models were trained over the Mixed kidney stone dataset.}
\label{table_accuracy_Losses_Functions}
\end{table*}

==> tables/table_Descriptors_example.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{}
\label{table_Descriptors}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccc}
\multicolumn{4}{c}{PPs 13th}                                             \\ \hline
\multicolumn{2}{c}{Local Analysis} & \multicolumn{2}{c}{Global Analysis} \\ \hline
Descriptor & \begin{tabular}[c]{@{}c@{}}Local \\      Act. \%\end{tabular} & Descriptor & \begin{tabular}[c]{@{}c@{}}Global \\      Act. \%\end{tabular} \\ \hline
\textbf{Hue}    & \textbf{62\%}    & \textbf{Hue}     & \textbf{34\%}    \\
Texture         & 61\%             & Texture          & 31\%             \\
Contrast        & 58\%             & Contrast         & 25\%             \\
Shape           & 57\%             & Shape            & 24\%             \\
Brightness      & 50\%             & Brightness       & 15\%             \\
Saturation      & 30\%             & Saturation       & 15\%             \\ \hline
Avg             & 53\%             & Avg              & 24\%            
\end{tabular}%
}
\end{table}

==> tables/table_explanation_example_correctWD.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{}
\label{tab:my-table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc}
\multicolumn{3}{c}{Highest Prototipical-Part} \\ \hline
\multirow{3}{*}{Descriptor} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Local \\      Activation \%\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Global\\      Activation\end{tabular}} \\
                 &              &             \\
                 &              &             \\ \hline
Contrast         & 65.7\%       & 51.8\%      \\
Hue              & 64.1\%       & 51.6\%      \\
Texture          & 54.7\%       & 29.1\%      \\
Shape            & 46.6\%       & 31.5\%      \\
Saturation       & 44.8\%       & 37.3\%      \\
Brightness       & 0.7\%        & 19.1\%      \\ \hline
Avg.             & 46.1\%       & 36.7\%     
\end{tabular}%
}
\end{table}
